Variance-Optimal Augmentation Logging for Counterfactual Evaluation in Contextual Bandits

Methods for offline A/B testing and counterfactual learning are seeing rapid adoption in search and recommender systems, since they allow efficient reuse of existing log data. However, there are fundamental limits to using existing log data alone, since the counterfactual estimators that are commonly used in these methods can have large bias and large variance when the logging policy is very different from the target policy being evaluated. To overcome this limitation, we explore the question of how to design data-gathering policies that most effectively augment an existing dataset of bandit feedback with additional observations for both learning and evaluation. To this effect, this paper introduces Minimum Variance Augmentation Logging (MVAL), a method for constructing logging policies that minimize the variance of the downstream evaluation or learning problem. We explore multiple approaches to computing MVAL policies efficiently, and find that they can be substantially more effective in decreasing the variance of an estimator than na\"ive approaches.

==> Offline Experimental Design Draft (ArXiV)/notation.tex <==
%\DeclareMathOperator{\ent}{S}
\DeclareMathOperator{\Ex}{\mathbb{E}}
\DeclareMathOperator{\Var}{\text{Var}}
\DeclareMathOperator{\Cov}{\text{Cov}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
%\newcommand{\Pr}{\text{Pr}}
\newcommand{\sign}{\text{sign}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calO}{\mathcal{O}}

\newcommand{\IPS}{\text{IPS}}
\newcommand{\BAL}{\text{BAL}}

\newcommand{\x}{{x}}                 % Context
\newcommand{\xRV}{{X}}               % Context Random Variable
\newcommand{\action}{{a}}                 % Action
\newcommand{\actionRV}{{A}}               % Action Random Variable
\newcommand{\reward}{{r}}                 % Reward
\newcommand{\rewardRV}{{R}}               % Reward Random Variable
\newcommand{\Util}{{U}}                 % Reward
\newcommand{\UtilIPS}{{\hat{U}^{\text{IPS}}}}                 % Reward

\newcommand{\old}{{log}}
\newcommand{\eval}{{aug}}
\newcommand{\target}{{tar}}

\newcommand{\policy}{\pi}
\newcommand{\policyspace}{\Pi}
\newcommand{\oldpolicy}{\pi_{\text{\old}}}
\newcommand{\targetpolicy}{\pi_{\text{\target}}}
\newcommand{\targetpolicyspace}{\policyspace_{\text{\target}}}
\newcommand{\evalpolicy}{\pi_{\text{\eval}}}
\newcommand{\blendedpolicy}{\pi_{\text{balanced}}}
\newcommand{\minvarpolicy}{\pi_{\text{minvar}}^{\text{IPS}}}
\newcommand{\prodpolicy}{\pi_{\text{prod}}}
\newcommand{\maxpolicy}{\pi_{\text{max}}}

\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\sqaren}[1]{\left[#1\right]}

\newcommand{\dataset}{\calD}
\newcommand{\evaln}{{n_\text{\eval}}}
\newcommand{\oldn}{{n_\text{\old}}}
\newcommand{\evalD}{{\dataset_\text{\eval}}}
\newcommand{\oldD}{{\dataset_\text{\old}}}


\newcommand{\rewardmean}{{\bar \reward(\x,\action)}}
\newcommand{\rewardmeansq}{{\bar \reward^2(\x,\action)}}
\newcommand{\rewardvar}{{\sigma^2(\x,\action)}}
\newcommand{\expectedsquarer}{\Ex_r\sqaren{r^2(x, a)}}
\newcommand{\expectedsquarertight}{\Ex_r\!\!\sqaren{r^2(x, a)}}

% If you go back to the old version, also remember to change optimization problem 2
\newcommand{\rewardmeansqprewardvar}{\expectedsquarer}
\newcommand{\parenrewardmeansqprewardvar}{\expectedsquarer}

\newtheorem{optimizationproblem}{Optimization Problem}


%%%%%%%%%%%%% Comments
\newcommand{\tj}[1]{\footnote{\textcolor{magenta}{TJ comments: #1}}}
\newcommand{\at}[1]{\footnote{\textcolor{blue}{AT comments: #1}}}


==> Offline Experimental Design Draft (ArXiV)/sections/conclusions_and_future.tex <==
\section{Conclusions}

We introduced and formalized the problem of augmentation logging, and derived MVAL as a principled and practical method for variance-optimal data gathering for off-policy evaluation. We extended the approach to multi-policy evaluation and batch learning, and find that it can substantially improve estimation and learning quality over naive methods. This work opens up a number of directions for future work. For example, contextual-bandit problems with combinatorial actions like slates \cite{slate} raise additional challenges, but they also provide structure that connects the observations for different actions. It is interesting to explore how this structure can inform augmentation logging for improved bias/variance trade-offs.
%Theoretically, MVAL provides a principled method for balancing different considerations in collecting data for policy evaluation, and in special cases agrees with intuitively reasonable choices. If a new action is introduced, then the best evaluation policy needs to play that action according to Theorem \ref{thm:newaction}. When there is no data available and no model of the reward variance $\Ex_r[r^2(x, a)] = \bar r^2(x, a) + \sigma^2(x, a)$, it uses the target policy for single policy evaluation according to Theorem \ref{thm:target}, or the uniform policy for evaluating the space of all valid policies according to Theorem \ref{thm:uniform}. Empirically, MVAL exhibits strong performance improvements for single policy evaluation, multiple policy evaluation, and even sequential policy learning.



%\subsection{Future work}
%\paragraph{Ambiguity set construction} The policy learning experiment was successful even with a simple policy class construction. In other work \cite{ucb}, the construction of an ambiguity class was a key element to achieving good exploration. Properly analyzing this problem is left to future work.

%\paragraph{Learning a model of $r(x, a)$ and $\sigma^2(x, a)$} Our experiments used a uniform value for $r(x, a)$ and $\sigma^2(x, a)$. MVAL is encouraged to choose actions with high reward, and with high variance. This is similar to encouraging exploration, and properly analyzing the problem is left to future work.

==> Offline Experimental Design Draft (ArXiV)/sections/empirical.tex <==
%\subsection{Experiment Setup}
%The experiments shared a few preliminary details.

%\paragraph{Dataset} 
To evaluate MVAL on a real-world contextual bandit problem, we performed experiments on the Yahoo!\ Front Page Dataset \cite{yahoodata}\footnote{\label{license}This dataset was obtained from Yahoo! Webscope at \url{http://research.yahoo.com/Academic_Relations}. \label{identifiable} The users are anonymized.}. Each context in the dataset consists of a $5$-dimensional vector $\mathbf u$ representing the user, as well as a $D\times 5$ dimensional matrix with vectors $\mathbf A_i$ for each of the $D$ articles. For convenience, we only used contexts with exactly $19$ articles. The dataset includes which article was recommended (i.e., the action) and if the user clicked on the article (i.e., the reward).

When collecting this dataset, the article recommendations were chosen uniformly at random from the articles available for the context. This allows for an unbiased simulation of running a different article recommendation policy $\pi$ using rejection sampling \cite{krause_yahoo}. To construct a sample for a new policy $\pi$, we iterate through the contexts $x_i$ and sample $a' \sim \pi(\cdot|x)$ according to $\pi$. If the $a'$ sampled from our policy agrees with the observed action $a_i$, we include that $(x_i, a_i, r_i)$ tuple. This gives us an unbiased sample that comes from the same distribution as if we were running our new policy $\pi$ on the operational system.
%TODO(Aaron) cite the replay methodology (probably from Yahoo paper)

%This simulates running our policy on the operational system, and it is an unbiased sample because $a_i$ is independent of both the context $x_i$ and our choice $a'$.



\vspace*{-1mm}\paragraph{Model Architecture and Training.}
%            Dense(256, activation='relu'),
%            Dense(256, activation='relu'),
%            Dense(64, activation='relu'),
%            Dense(1, activation='linear')
The policy architecture for precomputed MVAL is a feedforward neural network, ending in a softmax layer where the logit for article $j$ is based on the concatenation of the user vector to the article vectors $\mathbf u \circ \mathbf A_j$ passed through 2 fully connected ReLU \cite{relu} layers with $256, 256$ nodes before $1$ fully connected linear node. Adam is used for optimization with the standard parameters $\alpha=0.001$, $\beta_1=0.9$, $\beta_2=0.999$ \cite{adam} and a batch size of $10000$. All experiments can be run on a desktop with an RTX2080. \label{specs}

\vspace*{-1mm}\paragraph{Estimating $\rewardmeansqprewardvar$.} The first set of experiments use a uniform $\rewardmeansqprewardvar$, since these experiments explore how any decrease in variance is a result of the algorithmic improvement, rather than a result of a model of $\rewardmeansqprewardvar$. For the sequential learning experiment, we use a feedforward neural network to approximate $\Ex\sqaren{r^2(x,a)}$, trained using mean squared error to perform regression on the quantity $r^2(x,a)$ using the same architecture as the policy networks described above.

\vspace*{-1mm}\paragraph{Generating Logging and Target Policies.}\label{crosspolicy} 
The policy evaluation experiments use randomly generated target and logging policies.
We control the generating process to vary how deterministic the logging policy's actions are, and how different the target and logging policies are.
In particular, to generate the logging policy, we randomly sample a vector $\mathbf v \in \mathbb{R}^{25}$ such that $v_i \sim \mathcal{N}(\mu=0, \sigma=1)$. This vector is then multiplied against a feature vector of the cross terms between $u$ and each $A_i$ for the given context $i$ to allow for interactions between user and article features while remaining a simple policy class. Then, the articles are ranked according to this value to define the selection probabilities of the policy based on the rank. In particular, the probability of choosing each article is proportional to $\eta^{\text{rank}_i}$, where $\text{rank}_i$ is the rank of the $i$th article. This allows us to increase the determinism of the policy by increasing $\eta$. We use the same construction to generate a target policy, but shift a $\delta$ fraction of the probability weight from the top-ranked article under the logging policy to the article that is ranked second under the logging policy. Increasing $\delta$ allows us to increase the difference between the target and logging policy.

\begin{figure}[t]
\includegraphics[width=.47\textwidth]{images/eta.png}
\vspace*{-4mm}
\caption{Variance of the balanced estimator while holding $\delta=0.4$ and increasing values of $\eta$, which increases the determinism of the policies. 
Error bars are the standard error based on $20$ trials. 
Note the logarithmic y axis.
%Both variations of MVAL substantially outperformed using the target policy or uniform distribution as the evaluation policy.
}
\label{fig:eta}
\end{figure}

\begin{figure}[t]
\includegraphics[width=.47\textwidth]{images/delta.png}
\vspace*{-4mm}
\caption{Variance of the balanced estimator while holding $\eta=4$ and increasing values of $\delta$, which increases the difference between the logging and target policies.
Error bars are based on $20$ trials.
%Both variations of MVAL substantially outperformed using the target policy or uniform distribution as the evaluation policy, though all policies suffered as the disagreement was increased.
}
\label{fig:frac}
\end{figure}

\subsection{Single Policy Evaluation}
The first experiments explore the effectiveness of MVAL for evaluating a single target policy while varying $\eta$ and $\delta$ for the logging and target policy generation. The reported variance is the empirical variance of $50$ sampled value estimates for the target policy. Each value estimate is generated by first sampling $900$ data points from the logging policy. We then compare different augmentation logging policies that are allow to sample $100$ additional data point. Specifically, we compare MVAL and precomputed MVAL to using the target policy or the uniform policy for augmentation logging. Finally, we estimating the value of the target policy using the balanced estimator on all $1000$ data points. The standard error bars are based on of $20$ such runs for each parameter setting.

In Figure \ref{fig:eta}, we see that using MVAL substantially outperforms using the target policy or uniform policy for augmentation logging for a range determinism factors $\eta$. The difference $\delta$ between logging and target policy is fixed at $0.4$ in this experiment. At $\eta=0$, the logging policy is the uniform distribution, and all policies have similar performance. We find that precomputed MVAL performs comparable to MVAL over the whole range of $\eta$.

In Figure \ref{fig:frac}, we vary the value of $\delta$ while the determinism factor $\eta$ is fixed. Again, we find that using MVAL to generate the augmentation policy substantially outperforms using the target policy or uniform distribution for a broad range of settings. Increasing the change fraction $\delta$ decreases the performance of all methods as expected. At $\delta=1$, MVAL and target tie because the target policy is fairly deterministic, and per Proposition \ref{thm:deterministic} the target policy is the variance-optimal augmentation policy. At  $\delta=1$, precomputed MVAL performs worse than exact MVAL, possibly because it is training a policy based on $(x, a, r)$ tuples close to the logging policy rather than the quite different target.



\begin{figure}
\includegraphics[width=.47\textwidth]{images/kway.png}
\vspace*{-3mm}
\caption{Variance of multiple policy evaluation for 3 policies with determinism factor $\eta=4$ and change fraction $\delta=0.4$. Each box plot contains all the empirical variances of all 3 policy estimates, for $20$ trials of the full experiment.
}
\label{fig:kway}
\end{figure}

\subsection{Multiple Policy Evaluation}


The next experiment explores the effectiveness of MVAL for multi-policy evaluation. The policies for this experiment were generated as before with determinism factor $\eta=4$ and a difference between logging and target policy of $\delta=0.4$. However, the $3$ target policies were constructed by shifting $\delta$ fraction of the logging policy's top action's probability to the $2$nd, $3$rd, and $4$th actions. The experiment variance is the empirical variance of $100$ runs of using the balanced estimator to estimate the target policy reward. The round-robin strategy uses each target policy to sample $333$ augmentation data points, while the other strategies collected $999$ augmentation data points from the uniform or precomputed MVAL policy. The original logging policy provided $9001$ data points for a total of $10000$ contexts. %The Precomputed MVAL policy is fit using $250$ iterations over its available contexts. 
As shown in Figure \ref{fig:kway}, precomputed MVAL substantially outperforms the round-robin and uniform strategies.

\subsection{Policy Learning}
\begin{figure}
\includegraphics[width=.47\textwidth]{images/sbo.png}
\vspace*{-3mm}
\caption{Average cumulative reward for sequentially using naïve or MVAL augmentation logging at each iteration for $\tau=1$. Error bars are the standard error based on $50$ trials.}
\label{fig:sbo}
\end{figure}

The final experiment explores the effectivess of MVAL for policy learning over time, where we repeatedly gather $10000$ additional augmentation data points and retrain the model using POEM \cite{poem} with the balanced estimator as policy learner.
In the initial iteration we gather $10000$ data points from the uniform policy, following the optimal MVAL strategy in this situation according to Proposition \ref{thm:uniform}. After that, each iteration $t$ trains a policy $\pi^t$ using POEM \cite{poem} with the balanced estimator as policy learner. We compare using MVAL for augmentation logging to naively logging additional data from the target policy $\pi^t$ in each iteration. We use precomputed MVAL with $\rewardmeansqprewardvar = m^t(x, a)$, where $m^t$ approximates $\expectedsquarer$ using regression. Furthermore, we approximate $\maxpolicy \approx \pi^t$ as discussed in Section~\ref{sec:multipol}. For both the naive augmentation logging using $\pi^t$ and MVAL augmentation logging we train POEM for $1000$ epochs, which is more than sufficient for convergence. The POEM clipping parameter is set to $10000$, which is chosen to maximize the performance of the naive method. Figure \ref{fig:sbo} shows that augmentation logging via MVAL outperforms naively using the target policy for augmentation logging.


%The final experiment explores the effectivess of MVAL for policy learning over time, where we repeatedly gather $10000$ additional augmentation data points and retrain the model using POEM \cite{poem} with the balanced estimator as policy learner. We compare using MVAL for augmentation logging to naively logging additional data from the target policy $\pi^t$ in each iteration. Both methods start with a batch of data from the uniform policy, which coincides with the optimal MVAL strategy in this situation according to Theorem \ref{thm:uniform}.  Using MVAL in the following iterations, we consider the trust region $\Pi_{\pi^t}=\{\pi | \forall x,a: \pi(a|x) \in [\frac{1}{\tau}\cdot\pi^t(a|x),\tau\cdot \pi^t(a|x)]\}$ around the current target policy $\pi^t$ for multi-policy MVAL, where $\tau$ controls the size of the trust region. We find that any small value of $\tau$ provides similar overall performance, which is not surprising since the solution of OP\ref{op:mvalmulti} is invariant to $\tau$ as long as $\pi^t(a|x)\le \frac{1}{\tau}$. We use precomputed MVAL with $\rewardmeansqprewardvar = m^t(x, a)$, where $m^t$ approximated $\expectedsquarer$ using regression. For both the naive augmentation logging using $\pi^t$ and MVAL augmentation logging we train POEM for $1000$ epochs, which is more than sufficient for convergence. The POEM clipping parameter is set to $10000$, which is chosen to maximize the performance of the naive method. Figure \ref{fig:sbo} shows that augmentation logging via MVAL outperforms naively using the target policy for augmentation logging. 

%At epoch $t>0$ it learns a POEM policy $\pi^t$ trained using the balanced estimator for all data logged from epochs $t'<t$ \cite{poem}, as well as a reward model $m^t$ to predict $\Ex\sqaren{r^2(x,a)}$ using regression. The augmentation policy $\evalpolicy^t$ is trained using precomputed MVAL for evaluating the performance of $\pi^t$ using $m^t(x, a) = \bar r^2(x,a) + \sigma^2(x, a)$. That policy $\evalpolicy^t$ is then used to sample the data for epoch $t$. The baseline instead simply uses $\pi^t$  to sample data for epoch $t$. Each epoch has $10000$ contexts, with the POEM policies and reward models trained for $1000$ iterations through the data. The POEM IPS weights for $\pi^t$ were clipped at $10000$, chosen by tuning to maximize the performance of the baseline method. As shown in Figure \ref{fig:sbo}, sequential MVAL outperforms the POEM baseline as soon as it starts training on data gathered through MVAL.



==> Offline Experimental Design Draft (ArXiV)/sections/old_empirical.tex <==
In addition to the theoretical results detailed above, we demonstrate the effectiveness of MVAL for single policy evaluation, multi-policy evaluation, and policy learning on the Yahoo! Front Page dataset. This dataset is based on real-world recommendation data, with the crucial property that it was sampled at random \cite{yahoodata}, which allows for unbiased simulations of running a policy.

\subsection{Experiment Setup}
Before discussing the experiments, there are a few shared preliminary details.

\paragraph{Dataset} Each context in the Yahoo! Front Page dataset consists of a $5$-dimensional vector $\mathbf u$ representing the user, as well as a $D\times 5$ dimensional matrix with vectors $\mathbf A_i$ for each of the $D$ articles. For convenience, we only used contexts with exactly $19$ articles. The dataset includes which article was recommended and if the user clicked. \label{identifiable}The users are anonymized. \label{license}This dataset was obtained from Yahoo! Webscope at \url{http://research.yahoo.com/Academic_Relations} \cite{yahoodata}.

\paragraph{Rejection Sampling}
In the Yahoo! Front Page Dataset the article recommendations were chosen uniformly at random from articles available in the context \cite{yahoodata}. This allows for an unbiased simulation of running an article recommendation policy $\pi$ using rejection sampling. To construct a sample, iterate through each context $x_i$ and sample $a' \sim \pi(\cdot|x)$. If the $a'$ sampled from our policy agrees with the observed action $a_i$ then include that $(x_i, a_i, r_i)$ tuple. This samples from running our policy on the real data because $a_i = a'$. This is an unbiased sample because the observed choice $a_i$ is independent of both the context $x_i$ and our choice $a'$.

\paragraph{Uniform values for $\bar r^2(x, a) + \sigma^2(x, a)$} All experiments used a uniform $\bar r^2(x, a) + \sigma^2(x, a)$, showing that the decreased variance is a result of the algorithmic improvement, rather than a result of the model of $\bar r^2(x, a) + \sigma^2(x, a)$.

\paragraph{Model Architecture and Training} Unless otherwise mentioned, the policy architecture for MVAL is a feedforward neural network, ending in a softmax layer where the logit for article $j$ is based on the concatenation of the user vector to the article vectors $\mathbf u \circ \mathbf A_j$ passed through 4 fully connected ReLU layers with $256, 256, 64$ and $1$ nodes \cite{relu}. The architecture for POEM-learned policies is the same, but with a $256$d hidden layer with ReLU activation and Batch Normalization followed by a  fully connected layer to produce a $1$d logit output. Adam is used for optimization with the parameters $\alpha=0.001$, $\beta_1=0.9$, $\beta_2=0.999$  \cite{adam}. All experiments can be run on a desktop with an RTX2080. \label{specs}

\paragraph{Randomly Generated Policies}
\label{crosspolicy} For the policy evaluation experiments we randomly generated the target and logging policies. Each was generated by randomly sampling a vector $\mathbf v \in \mathbb{R}^{25}$ such that $v_i \sim \mathcal{N}(\mu=1, \sigma=0.3)$. This vector is used to generate logits for the policy by multiplying it against a feature vector of the cross terms between $u$ and each $A_i$ for the given context. This allows for interactions between user and article features, while remaining a simple policy class. A softmax was then used with temperature $10$ to ensure opinionated policies.

\paragraph{Ambiguity Sets} Two of our experiments required an ambiguity set $\Pi$ to be constructed around a learned policy $\pi^t$. In these experiments we used $\Pi = \{\pi: \pi(a|x) \leq 2\pi^t(a|x), \sum_{a\in\calA}\pi(a|x) = 1\}$. The $2$ was not tuned, and using better ambiguity sets is left to future work.

\subsection{Single Policy Evaluation}

The natural first question is whether or not MVAL is an effective strategy for policy evaluation in the batched feedback from logged bandit with data augmentation setting. We compare the variance of MVAL to several baselines on randomly generated target and logging policies.

\paragraph{Experimental Setup}
The main point of this experiment was to simulate many trials of using off-policy estimators to evaluate the expected reward of a policy. Each off-policy evaluation trial is based on running an off-policy estimator on $\oldn=4$ contexts rejection sampled under the logging policy $\oldpolicy$, and $\evaln=1$ context rejection sampled under the augmentation policy $\evalpolicy$. These policies were randomly generated as per the procedure above. The reported variance is the empirical variance of the target policy utility estimates based on $10000$ trials. For this experiment, we shuffled the contexts in the dataset in order to avoid issues with the changing base rate of clicks and articles in the dataset.

\paragraph{Methods Compared} In addition to the basic form of MVAL which generates a policy for each context $x$, we used several other augmentation strategies for comparison. Precomputed MVAL is trained on the $40000$ contexts points rejection sampled under $\oldpolicy$. Precomputed MVAL used $25$ training epochs over its whole dataset. MVAL used $25000$ training iterations for each context, since it learns a separate policy for each context with no information sharing between them. This experiment had $4$ baselines, based on using a uniform distribution or the target policy as the augmentation policy, combined with the IPS or balanced estimator for off-policy evaluation.

\begin{figure}
    \begin{minipage}{0.47\textwidth}
    \includegraphics[width=\textwidth]{images/old2/policycomparison.png}
    \caption{Comparing MVAL variance to alternative augmentation policy and estimator combinations.}
    \label{fig:singlepolicyeval}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/kway.png}
        \caption{Variance resulting from different augmentation strategies to evaluate a group of $3$ policies. Based on 3333 samples.}
        \label{fig:kway}
    \end{minipage}
\end{figure}

\paragraph{Results}
Figure \ref{fig:singlepolicyeval} shows that MVAL is an effective augmentation logging strategy for single policy evaluation. precomputed MVAL outperformed every baseline, including ones using the Balanced Estimator. This shows that MVAL is a more effective method for augmentation logging for single policy evaluation, and that this improvement is not simply the result of switching to a better off-policy estimator.

\subsection{Multi-policy Evaluation}
Our second experiment considers multi-policy evaluation by comparing Precomputed Multi-Policy MVAL to a round-robin sampling of each of the target policies in the policy class.

\paragraph{Experimental Setup}
%\paragraph{Target and Logging Policies}
The target and logging policies were generated according to the same method explained in section \ref{crosspolicy}. To accommodate the round-robin sampling, $\oldn$ was increased to $12$, and $\evaln$ was increased to $3$. We estimated the variance as the empirical variance of $3333$ trials.  This uses the same number of total contexts as in the previous experiment. The round-robin baseline constructed the $3$ augmentation contexts by using each of the $3$ target policies to sample $1$ context. The uniform baseline used the uniform distribution to sample the $3$ augmentation contexts.

\paragraph{Results}
The results shown in Figure \ref{fig:kway} demonstrate that precomputed MVAL is an effective strategy for evaluating multiple policies. It decisively beats the round-robin baseline, as well as outperforms the uniform policy baseline.

\begin{figure}
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/phase3.png}
        \caption{Reward received by using the argmax of the learned policy after using the given augmentation policy.}
        \label{fig:phase3}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/cumulativeclickp.png}
        \caption{Cumulative average score. Note that the dataset is nonstationary, and the reward of choosing randomly changes over time.}
        \label{fig:sequential}
    \end{minipage}
\end{figure}


\subsection{Policy Learning}
Our third and fourth experiment demonstrates the efficacy of MVAL for policy learning.

\subsubsection{Data Augmentation for Policy Learning}
\paragraph{Experimental Setup}
This experiment is separated into three phases, each with 10,000 contexts. Between each stage, a POEM policy is learned using 100 iterations through the data up to that point. This POEM policy used the same architecture as MVAL, and a weight clip of 100. The first phase is a uniform phase where every strategy observes uniformly sampled contexts. The second phase is a learning phase where each strategy uses the augmentation strategy to generate more contexts to observe. The third is an evaluation phase where we observe the reward of the learned POEM policy where the policy uses the argmax of its probabilities instead of sampling stochastically.

\paragraph{Results}
Using Precomputed MVAL during the augmentation stage resulted in the policy with the highest argmax reward, shown in Figure \ref{fig:phase3}. This shows that MVAL augmentation is a good strategy for learning high-qualty policies. However, MVAL resulted in lower reward during the learning phase, getting roughly $0.02$ instead of $0.03$. This is unsurprising, because the MVAL objective minimizes the variance of the estimator without reference to expected reward.

\subsubsection{Sequential Policy Learning}
Previously, the experiments have focused on single-step learning. Now, we present an experiment which shows the value of this method to learn a policy over time.

\paragraph{The baseline} At epoch $0$, the a uniform policy is used. At epoch $t>0$ the baseline uses POEM (described in \cite{poem}) with the balanced estimator to learn a policy $\pi^t$ from all data logged from epoch $t'<t$, and then samples another batch of data using policy $\pi^t$ (using the rejection sampling method for simulating the use of a policy). Each epoch has $2000$ contexts, and POEM is trained for $100$ iterations through the data.

\paragraph{Sequential MVAL} Sequential MVAL has the same basic structure, except that after learning the policy $\pi^t$, we use it as the target policy to construct a policy class $\Pi^t=\{\pi': \pi'(a|x) \leq 2\pi^t(a|x)\}$. We then use precomputed MVAL to find the best augmentation policy $\evalpolicy^t$ for minimizing the variance of any policy $\pi'\in\Pi^t$, and then use $\evalpolicy^t$ to sample the next batch of data. MVAL is trained for $100$ iterations through the data. Note that this ambiguity set is chosen primarily for simplicity.

\paragraph{Results} As shown in Figure \ref{fig:sequential}, MVAL outperforms the Naive baseline of simply using the learned policy $\pi^t$ at each epoch. When the experiment is continued for more iterations, the Naive baseline catches up. This suggests that MVAL is useful for learning in the earlier stages of the problem, but given enough data POEM learns a good policy. This makes sense because it is only trying to minimize the estimate variance, without any reference to the expected value of the policy. Our ambiguity set does nothing to account this fact. While designing a proper trust region is left for future work, MVAL outperforms simply running the policy in the early stages even with a simple choice of trust region, and with a uniform reward distribution model.

==> sections/old_empirical.tex <==
In addition to the theoretical results detailed above, we demonstrate the effectiveness of MVAL for single policy evaluation, multi-policy evaluation, and policy learning on the Yahoo! Front Page dataset. This dataset is based on real-world recommendation data, with the crucial property that it was sampled at random \cite{yahoodata}, which allows for unbiased simulations of running a policy.

\subsection{Experiment Setup}
Before discussing the experiments, there are a few shared preliminary details.

\paragraph{Dataset} Each context in the Yahoo! Front Page dataset consists of a $5$-dimensional vector $\mathbf u$ representing the user, as well as a $D\times 5$ dimensional matrix with vectors $\mathbf A_i$ for each of the $D$ articles. For convenience, we only used contexts with exactly $19$ articles. The dataset includes which article was recommended and if the user clicked. \label{identifiable}The users are anonymized. \label{license}This dataset was obtained from Yahoo! Webscope at \url{http://research.yahoo.com/Academic_Relations} \cite{yahoodata}.

\paragraph{Rejection Sampling}
In the Yahoo! Front Page Dataset the article recommendations were chosen uniformly at random from articles available in the context \cite{yahoodata}. This allows for an unbiased simulation of running an article recommendation policy $\pi$ using rejection sampling. To construct a sample, iterate through each context $x_i$ and sample $a' \sim \pi(\cdot|x)$. If the $a'$ sampled from our policy agrees with the observed action $a_i$ then include that $(x_i, a_i, r_i)$ tuple. This samples from running our policy on the real data because $a_i = a'$. This is an unbiased sample because the observed choice $a_i$ is independent of both the context $x_i$ and our choice $a'$.

\paragraph{Uniform values for $\bar r^2(x, a) + \sigma^2(x, a)$} All experiments used a uniform $\bar r^2(x, a) + \sigma^2(x, a)$, showing that the decreased variance is a result of the algorithmic improvement, rather than a result of the model of $\bar r^2(x, a) + \sigma^2(x, a)$.

\paragraph{Model Architecture and Training} Unless otherwise mentioned, the policy architecture for MVAL is a feedforward neural network, ending in a softmax layer where the logit for article $j$ is based on the concatenation of the user vector to the article vectors $\mathbf u \circ \mathbf A_j$ passed through 4 fully connected ReLU layers with $256, 256, 64$ and $1$ nodes \cite{relu}. The architecture for POEM-learned policies is the same, but with a $256$d hidden layer with ReLU activation and Batch Normalization followed by a  fully connected layer to produce a $1$d logit output. Adam is used for optimization with the parameters $\alpha=0.001$, $\beta_1=0.9$, $\beta_2=0.999$  \cite{adam}. All experiments can be run on a desktop with an RTX2080. \label{specs}

\paragraph{Randomly Generated Policies}
\label{crosspolicy} For the policy evaluation experiments we randomly generated the target and logging policies. Each was generated by randomly sampling a vector $\mathbf v \in \mathbb{R}^{25}$ such that $v_i \sim \mathcal{N}(\mu=1, \sigma=0.3)$. This vector is used to generate logits for the policy by multiplying it against a feature vector of the cross terms between $u$ and each $A_i$ for the given context. This allows for interactions between user and article features, while remaining a simple policy class. A softmax was then used with temperature $10$ to ensure opinionated policies.

\paragraph{Ambiguity Sets} Two of our experiments required an ambiguity set $\Pi$ to be constructed around a learned policy $\pi^t$. In these experiments we used $\Pi = \{\pi: \pi(a|x) \leq 2\pi^t(a|x), \sum_{a\in\calA}\pi(a|x) = 1\}$. The $2$ was not tuned, and using better ambiguity sets is left to future work.

\subsection{Single Policy Evaluation}

The natural first question is whether or not MVAL is an effective strategy for policy evaluation in the batched feedback from logged bandit with data augmentation setting. We compare the variance of MVAL to several baselines on randomly generated target and logging policies.

\paragraph{Experimental Setup}
The main point of this experiment was to simulate many trials of using off-policy estimators to evaluate the expected reward of a policy. Each off-policy evaluation trial is based on running an off-policy estimator on $\oldn=4$ contexts rejection sampled under the logging policy $\oldpolicy$, and $\evaln=1$ context rejection sampled under the augmentation policy $\evalpolicy$. These policies were randomly generated as per the procedure above. The reported variance is the empirical variance of the target policy utility estimates based on $10000$ trials. For this experiment, we shuffled the contexts in the dataset in order to avoid issues with the changing base rate of clicks and articles in the dataset.

\paragraph{Methods Compared} In addition to the basic form of MVAL which generates a policy for each context $x$, we used several other augmentation strategies for comparison. Precomputed MVAL is trained on the $40000$ contexts points rejection sampled under $\oldpolicy$. Precomputed MVAL used $25$ training epochs over its whole dataset. MVAL used $25000$ training iterations for each context, since it learns a separate policy for each context with no information sharing between them. This experiment had $4$ baselines, based on using a uniform distribution or the target policy as the augmentation policy, combined with the IPS or balanced estimator for off-policy evaluation.

\begin{figure}
    \begin{minipage}{0.47\textwidth}
    \includegraphics[width=\textwidth]{images/old2/policycomparison.png}
    \caption{Comparing MVAL variance to alternative augmentation policy and estimator combinations.}
    \label{fig:singlepolicyeval}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/kway.png}
        \caption{Variance resulting from different augmentation strategies to evaluate a group of $3$ policies. Based on 3333 samples.}
        \label{fig:kway}
    \end{minipage}
\end{figure}

\paragraph{Results}
Figure \ref{fig:singlepolicyeval} shows that MVAL is an effective augmentation logging strategy for single policy evaluation. precomputed MVAL outperformed every baseline, including ones using the Balanced Estimator. This shows that MVAL is a more effective method for augmentation logging for single policy evaluation, and that this improvement is not simply the result of switching to a better off-policy estimator.

\subsection{Multi-policy Evaluation}
Our second experiment considers multi-policy evaluation by comparing Precomputed Multi-Policy MVAL to a round-robin sampling of each of the target policies in the policy class.

\paragraph{Experimental Setup}
%\paragraph{Target and Logging Policies}
The target and logging policies were generated according to the same method explained in section \ref{crosspolicy}. To accommodate the round-robin sampling, $\oldn$ was increased to $12$, and $\evaln$ was increased to $3$. We estimated the variance as the empirical variance of $3333$ trials.  This uses the same number of total contexts as in the previous experiment. The round-robin baseline constructed the $3$ augmentation contexts by using each of the $3$ target policies to sample $1$ context. The uniform baseline used the uniform distribution to sample the $3$ augmentation contexts.

\paragraph{Results}
The results shown in Figure \ref{fig:kway} demonstrate that precomputed MVAL is an effective strategy for evaluating multiple policies. It decisively beats the round-robin baseline, as well as outperforms the uniform policy baseline.

\begin{figure}
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/phase3.png}
        \caption{Reward received by using the argmax of the learned policy after using the given augmentation policy.}
        \label{fig:phase3}
    \end{minipage}
    \hfill
    \begin{minipage}{0.47\textwidth}
        \includegraphics[width=\textwidth]{images/old2/cumulativeclickp.png}
        \caption{Cumulative average score. Note that the dataset is nonstationary, and the reward of choosing randomly changes over time.}
        \label{fig:sequential}
    \end{minipage}
\end{figure}


\subsection{Policy Learning}
Our third and fourth experiment demonstrates the efficacy of MVAL for policy learning.

\subsubsection{Data Augmentation for Policy Learning}
\paragraph{Experimental Setup}
This experiment is separated into three phases, each with 10,000 contexts. Between each stage, a POEM policy is learned using 100 iterations through the data up to that point. This POEM policy used the same architecture as MVAL, and a weight clip of 100. The first phase is a uniform phase where every strategy observes uniformly sampled contexts. The second phase is a learning phase where each strategy uses the augmentation strategy to generate more contexts to observe. The third is an evaluation phase where we observe the reward of the learned POEM policy where the policy uses the argmax of its probabilities instead of sampling stochastically.

\paragraph{Results}
Using Precomputed MVAL during the augmentation stage resulted in the policy with the highest argmax reward, shown in Figure \ref{fig:phase3}. This shows that MVAL augmentation is a good strategy for learning high-qualty policies. However, MVAL resulted in lower reward during the learning phase, getting roughly $0.02$ instead of $0.03$. This is unsurprising, because the MVAL objective minimizes the variance of the estimator without reference to expected reward.

\subsubsection{Sequential Policy Learning}
Previously, the experiments have focused on single-step learning. Now, we present an experiment which shows the value of this method to learn a policy over time.

\paragraph{The baseline} At epoch $0$, the a uniform policy is used. At epoch $t>0$ the baseline uses POEM (described in \cite{poem}) with the balanced estimator to learn a policy $\pi^t$ from all data logged from epoch $t'<t$, and then samples another batch of data using policy $\pi^t$ (using the rejection sampling method for simulating the use of a policy). Each epoch has $2000$ contexts, and POEM is trained for $100$ iterations through the data.

\paragraph{Sequential MVAL} Sequential MVAL has the same basic structure, except that after learning the policy $\pi^t$, we use it as the target policy to construct a policy class $\Pi^t=\{\pi': \pi'(a|x) \leq 2\pi^t(a|x)\}$. We then use precomputed MVAL to find the best augmentation policy $\evalpolicy^t$ for minimizing the variance of any policy $\pi'\in\Pi^t$, and then use $\evalpolicy^t$ to sample the next batch of data. MVAL is trained for $100$ iterations through the data. Note that this ambiguity set is chosen primarily for simplicity.

\paragraph{Results} As shown in Figure \ref{fig:sequential}, MVAL outperforms the Naive baseline of simply using the learned policy $\pi^t$ at each epoch. When the experiment is continued for more iterations, the Naive baseline catches up. This suggests that MVAL is useful for learning in the earlier stages of the problem, but given enough data POEM learns a good policy. This makes sense because it is only trying to minimize the estimate variance, without any reference to the expected value of the policy. Our ambiguity set does nothing to account this fact. While designing a proper trust region is left for future work, MVAL outperforms simply running the policy in the early stages even with a simple choice of trust region, and with a uniform reward distribution model.
